Experimental Studies of Top Quark Production

In this review article three promising aspects of top quark production are discussed: the charge asymmetry in top quark pair production, the search for resonant top quark pair production, and electroweak single top quark production. First, an overview of the theoretical predictions of top quark pair and single top quark production is given. Then, for each topic the general analysis strategy and improvements are exemplarily explained using selected analyses and are put into the context of the global status at the beginning of LHC Run II and progress in this field. The example analyses discussed in more detail in this article use data from the LHC experiment CMS and for the charge asymmetry studies also data from the Tevatron experiment CDF have been used.

==> sections/abstract_de.tex <==
%% LaTeX2e class for student theses
%% sections/abstract_de.tex
%% 
%% Karlsruhe Institute of Technology
%% Institute for Program Structures and Data Organization
%% Chair for Software Design and Quality (SDQ)
%%
%% Dr.-Ing. Erik Burger
%% burger@kit.edu
%%
%% Version 1.1, 2014-11-21

\Abstract
Deutsche Zusammenfassung

==> sections/content.tex <==
%% LaTeX2e class for student theses
%% sections/content.tex
%% 
%% Karlsruhe Institute of Technology
%% Institute for Program Structures and Data Organization
%% Chair for Software Design and Quality (SDQ)
%%
%% Dr.-Ing. Erik Burger
%% burger@kit.edu
%%
%% Version 1.1, 2014-11-21

\chapter{First Content Chapter}
\label{ch:FirstContent}

%% -------------------
%% | Example content |
%% -------------------
The content chapters of your thesis should of course be renamed. How many
chapters you need to write depends on your thesis and cannot be said in general.

Check out the examples theses in the SDQWiki:

\url{https://sdqweb.ipd.kit.edu/wiki/Abschlussarbeit/Studienarbeit}

Of course, you can split this .tex file into several files if you prefer. 


\section{First Section}
\label{sec:FirstContent:FirstSection}

\dots

\section{Second Section}
\label{sec:FirstContent:SecondSection}

\dots


\chapter{Second Content Chapter}
\label{ch:SecondContent}

\dots

\section{First Section}
\label{sec:SecondContent:FirstSection}

\dots

\section{Second Section}
\label{sec:SecondContent:SecondSection}

\dots

Add additional content chapters if required by adding new .tex files in the
\code{sections/} directory and adding an appropriate 
\code{\textbackslash include} statement in \code{thesis.tex}. 
%% ---------------------
%% | / Example content |
%% ---------------------

==> sections/declaration.tex <==
%% LaTeX2e class for student theses: Declaration of independent work
%% sections/declaration.tex
%% 
%% Karlsruhe Institute of Technology
%% Institute for Program Structures and Data Organization
%% Chair for Software Design and Quality (SDQ)
%%
%% Dr.-Ing. Erik Burger
%% burger@kit.edu
%%
%% Version 1.1, 2014-11-21

\thispagestyle{empty}
\null\vfill
\noindent\hbox to \textwidth{\hrulefill} 
\iflanguage{english}{I declare that I have developed and written the enclosed
thesis completely by myself, and have not used sources or means without
declaration in the text.}%
{Ich versichere wahrheitsgemäß, die Arbeit
selbstständig angefertigt, alle benutzten Hilfsmittel vollständig und genau
angegeben und alles kenntlich gemacht zu haben, was aus Arbeiten anderer
unverändert oder mit Änderungen entnommen wurde.}
 
 
%% ---------------------------------------------
%% | Replace PLACE and DATE with actual values |
%% ---------------------------------------------
\textbf{PLACE, DATE}
\todo{Please replace with actual values}
\vspace{1.5cm}
 
\dotfill\hspace*{8.0cm}\\
\hspace*{2cm}(\theauthor) 
\cleardoublepage

==> sections/evaluation.tex <==
%% LaTeX2e class for student theses
%% sections/evaluation.tex
%% 
%% Karlsruhe Institute of Technology
%% Institute for Program Structures and Data Organization
%% Chair for Software Design and Quality (SDQ)
%%
%% Dr.-Ing. Erik Burger
%% burger@kit.edu
%%
%% Version 1.1, 2014-11-21

\chapter{Evaluation}
\label{ch:Evaluation}

%% -------------------
%% | Example content |
%% -------------------
\dots

\section{First Section}
\label{sec:Evaluation:FirstSection}

\dots

\section{Second Section}
\label{sec:Evaluation:SecondSection}

\dots

\section{Third Section}
\label{sec:Evaluation:ThirdSection}

\dots
%% ---------------------
%% | / Example content |
%% ---------------------

==> sections/papers.tex <==
%\RequirePackage{xcolor}
%\definecolor{color1}{rgb}{0.35,0.70,0.30}% green

\chapter{Journal Articles of Habilitation Thesis}
\label{ch:papers}



\begin{enumerate}
\item{\textbf{Charge Asymmetry in Top Quark Pair Production:}}
\begin{enumerate}
\item{T.~Aaltonen et al.,  CDF Collaboration,
  ``Forward-Backward Asymmetry in Top Quark Production in $p\bar{p}$ Collisions at $\sqrt{s}=1.96\; \mbox{TeV}$'', Phys.Rev.Lett. 101, 202001 (2008), \textbf{(100+)}.}
\item{S.~Chatrchyan et al., CMS Collaboration, ``Inclusive and differential measurements of the $t\bar{t}$ charge asymmetry in pp collisions at 7 TeV'', Phys.Lett. B717, 129 (2012), \textbf{(50+)}.}
\item{S.~Chatrchyan et al., CMS Collaboration, ``Measurement of the charge asymmetry in top-quark pair production in proton-proton collisions at $\sqrt{s} = 7$ TeV'', Phys. Lett. B709, 28 (2012), \textbf{(50+)}.}
\end{enumerate}
\item{\textbf{Search for Resonant Top Quark Pair Production:}}
\begin{enumerate}
\item{S.~Chatrchyan et al., CMS Collaboration, ``Search for resonant $t\bar{t}$ production in lepton+jets events in pp collisions at $\sqrt{s}=7$ TeV'', JHEP 1212, 015 (2012), \textbf{(50+)}.}
\end{enumerate}
\item{\textbf{Experimental Studies of \boldmath{$t$}-Channel Single Top Quark Production:}}
\begin{enumerate}
\item{S.~Chatrchyan et al., CMS Collaboration, ``Measurement of the t-channel single top quark production cross section in pp collisions at $\sqrt{s} = 7$ TeV'', Phys.Rev.Lett. 107, 091802 (2011), \textbf{(100+)}.}
\item{S.~Chatrchyan et al., CMS Collaboration, ``Measurement of the single-top-quark t-channel cross section in pp collisions at $\sqrt{s} = 7$ TeV'', JHEP 1212, 035 (2012), \textbf{(100+)}.}
\end{enumerate}
\end{enumerate}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mttbar"
%%% End: 

